Structure of Core-Periphery Communities

It has been experimentally shown that communities in social networks tend to have a core-periphery topology. However, there is still a limited understanding of the precise structure of core-periphery communities in social networks including the connectivity structure and interaction rates between agents. In this paper, we use a game-theoretic approach to derive a more precise characterization of the structure of core-periphery communities.

==> content/algo.tex <==
\noindent{\underline{ Content Recommendation Algorithms:}}%\label{sec:rec_algos}
Content recommendation algorithms decide for each content consumer, the content that is recommended to the content consumer on each topic $k \in \setT$.
Formally, this decision is captured by the recommendation function  $\ind{a}{i}{b}{j}(k)$,
where $\ind{a}{i}{b}{j}(k) \in [0, 1]$ determines the fraction of content produced by a content producer $x \in \setP_i$ with interest range $a$,  that is recommended to a consumer with main interest $T_k$ and interest range $b$. 
%For example, the indicator $I(k|a,i)$ is equal to 1 if all of  the content on topic $T_k$ is recommended to a consumer with main interest $T_i$, and equal to $0$ if no content on topic $T_k$ is recommended to the consumer.
For our analysis we assume that there is a bound (capacity) of the amount of content a consumer can consume (read)  within a given time period, and we have that
$$ \sum_{i=-M}^M  \left [ \sum_{a \in \setA} N_p(a)  \left ( \sum_{k=-M}^M  \ind{a}{i}{b}{j}(k)  \right )  \right ] \leq L_c, \qquad j=-M,...,M,$$
where $L_c > 0$. We refer to $L_c$  as the recommendation capacity.

\noindent{\underline{Impact of Recommendation Function on Consumption and Production Utilities:}}
The consumption utility $\Ucons{b}(j)$ for content consumers with main interest $T_j$ and interest range $b$, is then given by
$$\Ucons{b}{j} = \sum_{i=-M}^M \left [ \sum_{a \in \setA} N_p(a)    \left ( \sum_{k=-M}^M \ind{a}{i}{b}{j}(k) \cprod{a}{i}(k) \funq{a}{i}(k) \funp{b}{j}(k)  \right )  \right ].$$
Similarly, the production utility of content producers with main interest $T_i$  and range of interest $a$ is given by
\begin{equation}\label{eq:uprod}
\Uprod{a}{i} = \sum_{j=-M}^M \left [ \sum_{b\in \setA} N_c(b)   \left ( \sum_{k=-M}^M \ind{a}{i}{b}{j}(k) \cprod{a}{i}(k) \funq{a}{i}(k) \funp{b}{j}(k)  \right )  \right ]. 
\end{equation}



\noindent{\underline{Impact of Recommendation Function on Content Producer:}}
In Eq.~\eqref{eq:uprod}, the utility of content producers with main interest $T_i$  and range of interest $a$ depends on the allocation $\cprod{a}{i}(k)$, and the recommendation function $\ind{a}{i}{b}{j}(k)$. Content producers have no control over (i.e. do not choose) the recommendation function $\ind{a}{i}{b}{j}(k)$. However, content producers with main interest $T_i$ decide on  production allocation $\cprod{a}{i}(k)$. This suggests to the following. For a given recommendation function, content producers with main interest $T_i$ and range of interest $a$ should choose an  allocation $\optcprodI{a}{i}$ that maximizes the content production utility given by Eq.~\eqref{eq:uprod}.
More formally, let
$$ \setB = \{ \cprodv \in [0,1]^M | \sum_{k=-M}^{M} \cprodv(k) \leq L_p\}.$$
be the set of all possible content production allocations that meet the production capacity constraint.
The goal of producers with main interest $T_i$ and range of interest $a$  is then to choose an allocation $\optcprod{a}{i} \in \setB$ that maximizes the content production utility, and we have that
$$ \optcprod{a}{i} = \arg\max_{\cprodv \in \setB} \Uprod{a}{i}.$$
%Let $\optcprod{I} = (\optcprodI{I}{-M},...,\optcprodI{I}{M})$ be the corresponding optimal allocation vector for all content producers.




==> content/applications.tex <==
\section{Applications}\label{sec:appl}
In Section~\ref{sec:structural_property} we derived structural properties of a core-periphery community. In this section we discuss how these results can be used to design algorithms for social networks. In particular, we discuss how the results can be used to design a) incentive mechanisms for social networking applications, b) algorithms for the early detection of viral content and community-based content recommendation, and c) community detection algorithms that require only local information. 







\subsection{Incentive Mechanisms for Social Networking Applications}\label{ssec:incentive}
A goal in the design of social networking  applications is to implement an application that leads to a high user engagement. However, there currently does not exist a formal understanding of how to achieve this design goal. As a result, social networking applications are designed  based on an intuitive understanding,  and different design options are tested and evaluated using  trial-and-error. However this approach to the design of social networking applications can be costly and time-consuming.  This gives raise to the  question whether there exists an alternative approach that is more systematic, i.e.  an approach that is based on a formal understanding of how to design social networking applications that lead to a high user engagement. Proposition~\ref{prop:core_influence} of Section~\ref{sec:structural_property} provides such an approach.  Proposition~\ref{prop:core_influence} states that the core agent has a direct influence on the user engagement: the more time the core agent allocates to aggregate content for periphery agents, the more time the periphery agents will allocate to the community, and the higher the user engagement will be.
This suggests that having mechanism that encourages core agents to allocate more time to the community, and to provide high quality content,  is an efficient way to increase user engagement. 
Indeed, existing social networking applications pursue this approach, and implement incentive mechanisms for users to allocate more time to the community, and provide high quality content. Existing incentive mechanisms include reputation, and monetary, based mechanisms. An example of a reputation based incentive mechanism is the follower score implemented by Twitter that encourages users to attract as many as followers as possible. An example of a monetary based mechanisms is the mechanism implemented by YouTube where users obtain a monetary reward based on the number of followers, and views, that their content attracts. 
While incentive mechanisms are already used and implemented in practice, there currently exists only a limited understanding of how to best design and implement such mechanisms.
One existing result that provides insight into how to design such an incentive mechanism is provided  by Jackson and Wolinsky. In~\cite{social_econ_game}, Jackson and Wolinsky derive  a mechanism  based on side payments, and show this mechanism can be used to provide the incentive for a core agent to aggregate content on behalf of the periphery agents~\cite{social_econ_game}. The analysis by Jackson and Wolinsky is  carried out for the special case of a homogeneous set of periphery agents. The model presented in this paper can be used to extend this analysis to the case of a heterogeneous set of periphery agents. Carrying out this analysis, and using it to provide a formal approach to design reputation based, as well as monetary based, incentive mechanisms for social networking applications is ongoing research. 





\begin{figure}
% \subfloat[Connectivity Structure for Content Produced by Periphery Agent.]
%        {\includegraphics[width = 0.5\linewidth]{result/information_propogation.png}} \quad
	%\subfloat[Information Flow of Content Produced by Periphery Agent.]
         {\includegraphics[width = 0.8\linewidth]{result/information_propogation2.png}} 
       \caption{Illustration of Broadcast Trees for Content Produced by a Periphery Agent.}
       %\caption{An Illustration of Information Propogation within Community. If we remove the content space and reposition the nodes, we would get a propogation structure that is closed to the ``broadcast'' observed in the experiment~\cite{broadcast}.}
	\label{fig:information_propogation}
\end{figure}

\subsection{Early Detection of Viral Content and Community-Based Content Recommendation}\label{ssec:diffusion}

Understanding how content propagates within a community, and a social network, has been  extensively studied~\cite{social_network_survey}. While initial propagation models were based on a cascade model, experimental results have shown that content propagation tends to follow a broadcast model rather than a cascade model~\cite{broadcast}. The structural properties obtained in Section~\ref{sec:structural_property} provide an approach to study content propagation in core-periphery communities in a formal manner. In particular, the results of Section~\ref{sec:structural_property} show  that content indeed propagates according to  broadcast model, where a content item that is produced by a periphery agent has two broadcast trees. First, the broadcast tree formed by other periphery agents (as given by Proposition~\ref{prop:periphery_local_interaction}) that follow the source agent directly. Second, the broadcast tree formed by the core agent that is followed by the remaining periphery agents in the community. Fig.~\ref{fig:information_propogation} illustrates these two broadcast trees. An interesting question is whether the result of   Proposition~\ref{prop:periphery_local_interaction} can be used to obtain a more precise characterization of how content is propagated within a community, and whether this characterization can be used  to determine a) which users in the community are most likely interested in a given content item, and b) whether a given content item is likely to propagate through the entire community. Such an analysis could be used to design algorithms for the early detection of popular/viral content within a community, as well as for community-based content recommendation. Using the result of Proposition~\ref{prop:periphery_local_interaction} to obtain a more precise characterization of content propagation, and the design of algorithms for the early detection of viral content and content recommendation, is ongoing research. 



\subsection{Community Detection using Local Information}\label{ssec:local_algo}
Proposition~\ref{prop:periphery_consumption} in Section~\ref{sec:structural_property} provides a ranking function for periphery agents. 
An application of this ranking function  is to  design a community detection algorithms that require only local information. More precisely, the ranking function given by Proposition~\ref{prop:periphery_consumption} can be used identify the ``center'' of a community in an iterative manner as follows. Starting with any periphery agent, the algorithm examines the local neighborhood of this agent and picks as the next agent the agent with the highest ranking according to the function given by Proposition~\ref{prop:periphery_consumption}. By Proposition~\ref{prop:periphery_consumption}, this new agent is the the agent in the local neighborhood that is closet to the center of the community. This algorithm allows to iteratively make progress towards identifying the agents in the center of the community.  Once the agents in the community center have been identified, these agents can be used as a seed set to identify the entire community by using  a community expansion algorithm such as~\cite{seed_set}. Of course, this algorithm needs  to be formulated and analyzed in a rigorous manner. In particular, the algorithm relies on being able to accurately estimate the ranking function of an agent based on observable data, and showing that these estimates will indeed result in an agent that is closer to the center of the community at each iteration step. The design and analysis of such an algorithm  is ongoing research.

%\subsection{Hierarchical Community Structure}
%In this paper we focus on studying  a single community.
%In social networks, communities are typically embedded in a hierarchical structure. That is, small communities build larger ones, which in turn group together to form even larger ones, etc.  Extending the model of Section~\ref{sec:model} to study the stability and efficiency, as well as the structural properties, of hierarchical community structures  is future research. Beyond allowing to characterize and understand the connectivity structure, such an analysis could also be used to characterize the  information flow (between communities), in a social network with a hierarchical community structure. The results of such an analysis could potentially also be used to design and analyze community detection algorithms that are able to ``reconstruct'' the underlying structure of a hierarchical social network.

%\subsection{Community Formation Process}\label{ssec:formation}



==> content/case_study.tex <==
\section{Numerical Case Study}\label{sec:case_study}

\subsection{Static Population}




\subsection{Dyanmic Population}



\subsection{Discussion}


==> content/intro.tex <==
\section{Introduction}\label{sec:intro}

Social media allows for a wide variety of content to be published both in terms of the diversity of topics that are covered, as well as the diversity of users who produce the content. The diversity of the users who produce content can be measured along several dimensions, in this paper we focus on the range of interests that content producers have, i.e. whether content producers have a more narrow range of interests, or a broader range of interest. One may think of the former type as specialists, or experts, and the latter as generalists.

The question that we study is whether, and how, social media content recommendation algorithms impact the population of content producers, and content consumers, in terms of the range of interest of the population of content producers and consumers. To do that, we consider three different content recommendation algorithms, with different content recommendation objectives, and characterize the population of content producers and consumers under the different recommendation algorithms.

Our results show that content recommendation algorithms indeed impact the population of content producers and consumers. The results of our analysis have the following implications:
%\begin{enumerate}
%\item[a)]
first, they show that content recommendation algorithms impact more than just the content that is being recommended to content producers, and they also impact the population of content producers and consumers that are attracted, and active, on social media platforms, and
%\item[b)]
second, they show the impact of content recommendation algorithms it not that straightforward to model and understand, and the obtained results are not obvious, and
third, the understanding of the impact of recommendation algorithms on the user population is critical in order to understand the societal impact, such as polarization, of recommendation algorithms.
%\end{enumerate}



\section{Related Work}
The question studied in this paper is motivated by trying to understand the societal impact of content recommendation algorithms. In particular, the impact of recommendation algorithms on polarization.


There is concern that recommendation algorithms play a role in an increased degree of  polarization. In particular, there is a concern that social media content recommendation algorithms lead to echo chamber~\cite{Sunstein} and filter bubbles~\cite{Pariser}, which in return can lead to increased polarization on social media, and potentially within societies.  
However existing studies are not conclusive on  whether increased polarization in social media is caused a) by recommendation algorithms through the creation of echo chambers~\cite{..}, or b) by (new) users who join recommendation algorithms. For the latter, the argument is that (independent from recommendation algorithms) that increased polarization is created by users with ``extreme'', or polarized,  viewpoints who join social media platforms~\cite{..}. 
Below be provide an overview of existing studies of how recommendation algorithms, and the user population, impact polarization.
%The motivation for this users to join social media platforms could be external events (such as a political election cycle)~\cite{Waller}, or the fact that the users identify more strongly with an issues and as a result are more motivated to be active, and vocal, on social media~\cite{McEwan}.

In this paper, we study the question whether in fact both arguments are valid in the sense that social media recommendation algorithms impact the population of users  who are active on  social media. If this is indeed the case, then this would suggest that social media recommendation algorithms impact polarization in two ways: first, through the creation of echo chambers, and second (and maybe more importantly) by affecting the mix of content producers and consumers on social media.



\vspace{-0.1in}
\paragraph{\bf Impact of Recommendation Algorithms on Polarization:}
Kitchens et al.  define in~\cite{Kitchens} polarization as "individual and collective adoption of more extreme views" and study the impact recommendation algorithm has on polarization with respect to the political dimension. To do that, they  analyze web browsing data of individual users on the three social media platforms Facebook, Reddit and Twitter. They characterize polarization in terms of a partisan shift i.e. to which degree users visit mostly news sites that correspond to either the most left-leaning, or most right-leaning, political viewpoints. Using this measure, they found that Facebook usage is correlated with an increase in the partisan shift, Reddit usage is correlated with a decrease, and Twitter usage has no significant impact on the partisan shift. 

Flaxman et al.  study in~\cite{Flaxman} how recent technological changes including search engines and social media impact polarization in the political dimension analyzing web browsing data of online news readers.
They found that social media leads to echo chambers and filter bubbles (reduced common content among users), but that the reduction in common content has limited impact on polarization~\cite{Flaxman}.

\vspace{-0.1in}
\paragraph{\bf Impact of User Population on Polarization:}
Waller and Anderson study political polarization on Reddit~\cite{Waller}, found that increased level of political polarization on Reddit was due to the arrival of new users, rather than existing users becoming more polarized. Their studies suggest that political polarization on Reddit is unrelated to previous activity on the platform, and is instead temporally aligned with external events. 

McEwan studies in~\cite{McEwan} .....


==> content/introduction.tex <==

\section{Introduction}\label{sec:intro}

Experimental results have shown that communities in social networks tend to have a core-periphery topology consisting of  two types of agents, core agents and periphery agents, that differ in their objectives for participating in the community~\cite{core_periphery_community_experiment,vlog}.
The objective of periphery agents is to obtain content that is of interest to them. As a result, periphery agents follow other agents in the community to obtain the content that is of most interest to them. 
The objective of the core agents is to attract followers, and attention, from the periphery agents. To achieve their objective, core agents aggregate/collect content from the community and make it available to the periphery agents~\cite{media_aggregate,jordan2012lattice,link_aggregator}.
These two different objectives lead to a community structure where the core agents follow periphery agents in the community in order to collect content,  and the periphery agents connect with the core agents and other periphery agents in order to obtain the content they are interested in~\cite{core_periphery_community_experiment,vlog}.

In this paper, we provide a mathematical model that allows us to derive these structural properties of core-periphery communities in social networks in a formal manner.
The results of our analysis provide a precise characterization of the connectivity structure, and interactions rates, of core-periphery communities.
%This allows us to use the structural properties to formally design algorithms for social networks such as (core-periphery) community detection algorithms, and content recommendation algorithms based on the users' interaction with a content item.  

For our analysis,  we use a game-theoretic framework where we assume that agents in the community make the decision on which other agents to interact with in a manner that maximizes their own objective.

Due to space constraints, we state our results without proofs. The proofs are provided in~\cite{technical}.



==> content/lemma/lemmaconcavity.tex <==
\begin{lemma}\label{lemma:concavity}
    Under assumption \ref{concave_assumption}, the optimization problems that characterize core and periphery agent's allocation are concave.
\end{lemma}
\begin{proof}
Let's consider the delay factor $e^{-\frac{\alpha}{\mu}}$ and denote it as $D(\mu)$. To show this lemma, it is enough to show $D(\mu)$ is concave, since the objectives function of core and periphery agents are sum of delay factor up to difference of a constant factor and the sum of concave function is again concave.


The first and second derivative of the delay factor are computed as follow:
\begin{equation}
    \begin{split}
        \frac{dD(\mu)}{d\mu} &= \frac{\alpha}{\mu^2}e^{-\frac{\alpha}{\mu}}\\
        \frac{d^2D(\mu)}{d^2\mu} &= \frac{\alpha}{\mu^3}e^{-\frac{\alpha}{\mu}}(\frac{\alpha}{\mu}-2)
    \end{split}
\end{equation}
By assumption \ref{concave_assumption}, we have $\mu > \frac{\alpha}{2}$, which leads to $\frac{d^2D(\mu)}{d^2\mu} < 0$. Therefore, the delay factor is concave in the region we are considering the interaction.
\end{proof}

==> content/lemma/lemmacore_agent_allocation.tex <==
\begin{lemma}\label{lemma:core_allocation}
If $b_c$ satisfy the condition in lemma \ref{lemma:periphery_agent_allocation},
then for arbitrary agents $y_i, y_j$ in the community such that
$$\|y_i - \Icen \| < \|y_j - \Icen \|$$
we have 
$$\mu(y_i|y_0) > \mu(y_j|y_0)$$
\end{lemma}

\begin{proof}
Let $y_i$, $y_j$ be two arbitrary agents such that 
$$\|y_i-y_0\| < \|y_j-y_0\|$$
To show the result of this lemma, it is enough to show the following
\begin{equation}\label{eq:lemma4_sufficient_condition}
    \sum_{z \in \Com \backslash \{y_i\}} B(y_i|z)e^{\frac{-\alpha}{\mu(y_0|z)}}> \sum_{z \in \Com \backslash \{y_j\}} B(y_j|z)e^{\frac{-\alpha}{\mu(y_0|z)}}
\end{equation}
then, first order condition condition would imply the optimal allocation has 
$$\mu(y_i|y_0) > \mu(y_j|y_0)$$


Recall $\delta$ is the distance of any consecutive agents in the content space of the community and it determine the community density. As $\delta$ decrease, the community density increase.
In addition, under the case without delay, by assumption \ref{assump:production_strategy}, we have that 
$ \sum_{z \in \Com \backslash \{y_i\}} B(y_i|z)> \sum_{z \in \Com \backslash \{y_j\}} B(y_j|z)$. Therefore, this lemma aim to establish that under the condition described, this relation is also true for the case with delay. To show this, we will use the result established in lemma \ref{lemma:periphery_agent_allocation},i.e. $\mu(y_0|y_i) > \mu(y_0|y_j)$. Using these results, we partition the community content interval and compare the utility of agents in each section. We will see that so long as the community is dense enough ($\delta$ small enough), then we obtain the relation in equation \ref{eq:lemma4_sufficient_condition}.


Let $\muc^*$ be the rate allocation vector of agents defined earlier. Without loss of generality, let's assume that content interval of the community is given by the following
$$I_C = (-L_C, L_C) \mbox{ and } mid(I_C) = 0$$
Then$\|y_i-\Icen \| < \|y_j-\Icen \|$ leads to three possible cases:\\
case 1: $y_i$ and $y_j$ are in the same side of the community, (0,$L_C$)\\
case 2: $y_i$ and $y_j$ are in the same side of the community, ($-L_C$,0)\\
case 3: $y_i$ and $y_j$ are on different side of the community


The proof for these three cases are similar. Therefore, we will only construct proof for one of the case above. Let's consider the case $y_i$, and $y_j$ are on the same half interval, (0,$L_C$). We can partition the community interval into the following sections:\\
\begin{equation*}
    \begin{split}
        S_1 &= (x^*(y_j),L_C)\\
        S_2 &= (\frac{x^*(y_j)-x^*(y_i)}{2},x^*(y_j))\\
        S_3 &= (x^*(y_i),\frac{x^*(y_j)-x^*(y_i)}{2})\\
        S_4 &= (x^*(y_i)+x^*(y_j)-L_C,x^*(y_i))\\
        S_5 &= (-L_C,x^*(y_i)+x^*(y_j)-L_C)
    \end{split}
\end{equation*}
Then, let's consider the difference of utility in each sections above.\\
Let $N(S_i)$ denote the set of leaf agents in the interval $S_i$, $\|N(S_i)\|$ is the number of leaf agents in $S_i$, and let $\Delta_{S_i}$ denote the difference of utility between $y_i$ and $y_j$ in interval $S_i$. Further, the $\Delta_{S_i}$ is given by 
\begin{equation*}
    \begin{split}
        \Delta_{S_i} &=\sum_{z \in N(S_i)} [B(y_i|z)-B(y_j|z)|z)] e^{-\frac{\alpha}{\mu(y_0|z)}} \\
        &= \sum_{z \in N(S_i)} [g(x^*(y_i)|y_i)f(x^*(y_i)|z)-\\
        &\hspace{0.5inch} g(x^*(y_j)|y_i)f(x^*(y_j)|z)] e^{-\frac{\alpha}{\mu(y_0|z)}} 
    \end{split}
\end{equation*}

We will show that the overall difference of $\Delta_{S_4}$ and $\Delta_{S_1}$ is positive,i.e,
$$\Delta_{S_4} + \Delta_{S_1} > 0$$

We know that the distance between consecutive agent is the same on the interval, and by construction, we have
$$\|S_1\| = \|S_4\|$$
which implies 
$$\|N(S_1)\| = \|N(S_4)\|$$
Let $J = \|N(S_1)\| = \|N(S_4)\|$. By construction of the information community in section \ref{sec:background} and the production strategy of agent \ref{assump:production_strategy}, we know that the distance between $x^*(y_j)$ to agents in $S_1$ are multiple of $\delta$ in addition to some distance $\epsilon_{s_1}$ to the first agent, where $\epsilon_{s_1} < \delta$.
Similarly for $S_4$. We can rewrite $\Delta_{S_1}$ and $\Delta_{S_4}$ as 
\begin{equation*}
    \begin{split}
        \Delta_{S_1} &= - \sum_{k=0}^J [g(x^*(y_j)|y_j)f(k\delta + \epsilon_{s_1} )\\
        &-g(x^*(y_i)|y_i)f(x^*(y_j)-x^*(y_i)+k\delta + \epsilon_{s_1}) ]e^{-\frac{\alpha}{\mu(y_0|x^*(y_j)+k\delta + \epsilon_{s_1})}}
    \end{split}
\end{equation*}
\begin{equation*}
    \begin{split}
        \Delta_{S_4} &= \sum_{k=0}^J [g(x^*(y_i)|y_i)f(k\delta + \epsilon_{s_4})\\
        &-g(x^*(y_j)|y_j)f(x^*(y_j)-x^*(y_i)+k\delta + \epsilon_{s_4})] e^{-\frac{\alpha}{\mu(y_0|x^*(y_i)-k\delta + \epsilon_{s_4})}}
    \end{split}
\end{equation*}

Then, with the result from assumption \ref{assump:production_strategy}, we have 
$$g(x^*(y_i)|y_i) > g(x^*(y_j)|y_j)$$
and by lemma \ref{lemma:periphery_agent_allocation}, we have that
$$e^{-\frac{\alpha}{\mu(y_0|x^*(y_j)+k\delta \pm \epsilon_{s_1})}}<e^{-\frac{\alpha}{\mu(y_0|x^*(y_i)-k\delta\pm \epsilon_{s_4})}}$$

Since $\epsilon_{s_1}, \epsilon_{s_4} < \delta$, we can make $\delta$ small enough such that the small misalignment $\epsilon_{s_1}, \epsilon_{s_4}$ does not effect the comparison of each term in the sum. Let $\delta_0$ be be the term that satisfy this condition. In other word, if $\delta < \delta_0$, then we have the following for each term of the two sum
\begin{equation*}
    \begin{split}
        &[g(x^*(y_i)|y_i)f(k\delta \pm \epsilon_{s_4})\\
        &-g(x^*(y_j)|y_j)f(x^*(y_j)-x^*(y_i)+k\delta + \epsilon_{s_4})] e^{-\frac{\alpha}{\mu(y_0|x^*(y_i)-k\delta + \epsilon_{s_4})}} \\
        &>\\
        &[g(x^*(y_j)|y_j)f(k\delta + \epsilon_{s_1} )\\
        &-g(x^*(y_i)|y_i)f(x^*(y_j)-x^*(y_i)+k\delta + \epsilon_{s_1}) ]e^{-\frac{\alpha}{\mu(y_0|x^*(y_j)+k\delta + \epsilon_{s_1})}}
    \end{split}
\end{equation*}


This means that each term in $\Delta_{S_4}$ is strictly larger than its corresponding term in $\Delta_{S_1}$. Therefore, we have
\begin{equation}\label{s14}
    \Delta_{S_1} + \Delta_{S_4} > 0    
\end{equation}

By similar argument, we can get
\begin{equation}\label{s23}
    \Delta_{S_2} + \Delta_{S_3} > 0    
\end{equation}

Now, let's consider the last interval $S_5$
\begin{equation*}
    \begin{split}
        \Delta_{S_5} &= \sum_{z \in N(S_5)} [B(y_i|z)-B(y_j|z)]e^{-\frac{\alpha}{\mu(y_0|z)}} 
    \end{split}
\end{equation*}
Since $y_i$ is closer to agents in $N(S_5)$ than $y_j$ by construction, we have 
$$B(y_i|z) > B(y_j|z) \text{  ,   } \forall z \in N(S_5)$$
This immediately leas to, 
\begin{equation}\label{s5}
    \Delta_{S_5} > 0
\end{equation}

Combining the results \ref{s14}, \ref{s23}, \ref{s5} above, we get
$$\Delta_{S_1}+\Delta_{S_2}+\Delta_{S_3}+\Delta_{S_4}+\Delta_{S_5}>0$$
Therefore, we obtain 
\begin{equation*}
    \sum_{z \in \Com \backslash \{y_i\}} B(y_i|z)e^{\frac{-\alpha}{\mu(y_0|z)}}> \sum_{z \in \Com \backslash \{y_j\}} B(y_j|z)e^{\frac{-\alpha}{\mu(y_0|z)}}
\end{equation*}
And the result of the lemma is immediately followed from first order condition.


\end{proof}

==> content/lemma/lemmacore_respond.tex <==
\newpage
\begin{lemma}\label{lemma:core_respond}
	If the set allocation of all periphery agents $\muc^*_p$ has the property that
	for agents $y_1, y_2$ in the community such that
	$$\mu(y_c|y_1) > \mu(y_c|y_1)$$
	if 
	$$\|y_1 - \Icen \| < \|y_2 - \Icen \|$$
	then, there exist a constant $\delta_2$, if the community density $\delta < \delta_2$, we have
	$$\mu(y_1|y_c) > \mu(y_2|y_c)$$
\end{lemma}

\begin{proof}
Let $y_1$, $y_2$ be two arbitrary agents such that 
$$\|y_1-\Icen\| < \|y_2-\Icen\|$$
To show the result of this lemma, it is enough to show the following
\begin{equation}\label{eq:lemma4_sufficient_condition}
    \sum_{z \in \Com \backslash \{y_1\}} B(y_1|z)e^{\frac{-\alpha}{\mu(y_c|z)}}> \sum_{z \in \Com \backslash \{y_2\}} B(y_2|z)e^{\frac{-\alpha}{\mu(y_c|z)}}
\end{equation}
then, first order condition condition would imply the optimal allocation has 
$$\mu(y_1|y_c) > \mu(y_2|y_c)$$


Recall $\delta$ is the distance of any consecutive agents in the content space of the community and it determine the community density. As $\delta$ decrease, the community density increase.
In addition, under the case without delay, by Proposition \ref{prop:production_strategy}, we have that 
$ \sum_{z \in \Com \backslash \{y_1\}} B(y_1|z)> \sum_{z \in \Com \backslash \{y_2\}} B(y_2|z)$. Therefore, this lemma aim to establish that under the condition described, this relation is also true for the case with delay. Using these results, we partition the community interval and compare the utility of agents in each section. We will see that so long as the community is dense enough ($\delta$ small enough), then we obtain the desired result


Let $\muc^*_p$ be the rate allocation vector of agents defined earlier. Without loss of generality, let's assume that content interval of the community is given by the following
$$I_C = (-L_C, L_C) \mbox{ and } mid(I_C) = 0$$
Then$\|y_1-\Icen \| < \|y_2-\Icen \|$ leads to three possible cases:\\
case 1: $y_1$ and $y_2$ are in the same side of the community, (0,$L_C$)\\
case 2: $y_1$ and $y_2$ are in the same side of the community, ($-L_C$,0)\\
case 3: $y_1$ and $y_2$ are on different side of the community


The proof for these three cases are similar. Therefore, we will only construct proof for one of the case above. Let's consider the case $y_1$, and $y_2$ are on the same half interval, (0,$L_C$). We can partition the community interval into the following sections:\\
\begin{equation*}
    \begin{split}
        S_1 &= (x^*(y_2),L_C)\\
        S_2 &= (\frac{x^*(y_2)-x^*(y_1)}{2},x^*(y_2))\\
        S_3 &= (x^*(y_1),\frac{x^*(y_2)-x^*(y_1)}{2})\\
        S_4 &= (x^*(y_1)+x^*(y_2)-L_C,x^*(y_1))\\
        S_5 &= (-L_C,x^*(y_1)+x^*(y_2)-L_C)
    \end{split}
\end{equation*}
Then, let's consider the difference of utility in each sections above.\\
Let $N(S_i)$ denote the set of leaf agents in the interval $S_i$, $\|N(S_i)\|$ is the number of leaf agents in $S_i$, and let $\Delta_{S_i}$ denote the difference of utility between $y_1$ and $y_2$ in interval $S_i$. Further, the $\Delta_{S_i}$ is given by 
\begin{equation*}
    \begin{split}
        \Delta_{S_i} &=\sum_{z \in N(S_i)} [B(y_1|z)-B(y_2|z)|z)] e^{-\frac{\alpha}{\mu(y_c|z)}} \\
        &= \sum_{z \in N(S_i)} [g(x^*(y_1)|y_1)f(x^*(y_1)|z)-\\
        &\hspace{0.5in} g(x^*(y_2)|y_1)f(x^*(y_2)|z)] e^{-\frac{\alpha}{\mu(y_c|z)}} 
    \end{split}
\end{equation*}

We will show that under some density, the overall difference of $\Delta_{S_4}$ and $\Delta_{S_1}$ is positive,i.e,
$$\Delta_{S_4} + \Delta_{S_1} > 0$$

We know that the distance between consecutive agent is the same on the interval, and by construction, we have
$$l = \|S_1\| = \|S_4\|$$
which implies 
$$\|N(S_1)\| = \|N(S_4)\|$$
Let $J = \|N(S_1)\| = \|N(S_4)\|$. By construction of the information community in Section \ref{sec:background} and the production strategy of agent \ref{prop:production_strategy}, we know that the distance between $x^*(y_2)$ to agents in $S_1$ are multiple of $\delta$ in addition to some distance $\epsilon_{s_1}$ to the first agent, where $\epsilon_{s_1} < \delta$.
Similarly for $S_4$. We can rewrite $\Delta_{S_1}$ and $\Delta_{S_4}$ as 


\begin{equation}\label{eq:s1_production}
    \begin{split}
        \Delta_{S_1} &= - \sum_{k=0}^J [g(x^*(y_2)|y_2)f(k\delta + \epsilon_{s_1} )\\
        &-g(x^*(y_1)|y_1)f(x^*(y_2)-x^*(y_1)+k\delta + \epsilon_{s_1}) ]e^{-\frac{\alpha}{\mu(y_c|x^*(y_2)+k\delta + \epsilon_{s_1})}}
    \end{split}
\end{equation}
\begin{equation}\label{eq:s4_production}
    \begin{split}
        \Delta_{S_4} &= \sum_{k=0}^J [g(x^*(y_1)|y_1)f(k\delta + \epsilon_{s_4})\\
        &-g(x^*(y_2)|y_2)f(x^*(y_2)-x^*(y_1)+k\delta + \epsilon_{s_4})] e^{-\frac{\alpha}{\mu(y_c|x^*(y_1)-k\delta + \epsilon_{s_4})}}
    \end{split}
\end{equation}

Then, with the result from Proposition \ref{prop:production_strategy}, we have 

\begin{equation}
	g(x^*(y_1)|y_1) > g(x^*(y_2)|y_2)
\end{equation}


and by assumption in this lemma, we have that for all $k$
\begin{equation}
	e^{-\frac{\alpha}{\mu(y_c|x^*(y_2)+k\delta + \epsilon_{s_1})}}<e^{-\frac{\alpha}{\mu(y_c|x^*(y_1)-k\delta+ \epsilon_{s_4})}}
\end{equation}

Consider the sum of each term of the Eq. \eqref{eq:s1_production} and \eqref{eq:s4_production} and to simply the notations in the analysis, let's make the following assignments

\begin{equation}
	\begin{aligned}
		&g(x^*(y_1)|y_1) = g_1\\
		&g(x^*(y_2)|y_2) = g_2\\
		&x^*(y_2)-x^*(y_1) = d\\
		&\mu(y_c|x^*(y_1)-k\delta + \epsilon_{s_4}) = \mu(x^*(y_1)-k\delta + \epsilon_{s_4})
	\end{aligned}
\end{equation}



\begin{equation}
    \begin{aligned}
        &[g_1 f(k\delta + \epsilon_{s_4})\\
        &-g_2|y_2)f(d+k\delta + \epsilon_{s_4})] e^{-\frac{\alpha}{\mu(x^*(y_1)-k\delta + \epsilon_{s_4})}} \\
        &-\\
        &[g_2|y_2)f(k\delta + \epsilon_{s_1} )\\
        &-g_1f(d+k\delta + \epsilon_{s_1}) ]e^{-\frac{\alpha}{\mu(x^*(y_2)+k\delta + \epsilon_{s_1})}}\\
        &>\\
        &([g_1f(k\delta + \epsilon_{s_4}) -g_2f(d+k\delta + \epsilon_{s_4})] \\
        &-[g_2f(k\delta + \epsilon_{s_1} )-g_1f(d+k\delta + \epsilon_{s_1})]) e^{-\frac{\alpha}{\mu(x^*(y_1)-k\delta + \epsilon_{s_4})}}\\
        &> \text{(first order condition of convex function)}\\
        &(g_1 - g_2)[f(k\delta)+f(d+k\delta) - O(\epsilon_{s_1})-O(\epsilon_{s_4})]*\\
        &e^{-\frac{\alpha}{\mu(x^*(y_1)-k\delta + \epsilon_{s_4})}} \\
        &>\text{(f is a decreasing function)}\\
        &(g_1 - g_2)[f(l)+f(d+l) - O(\epsilon_{s_1})-O(\epsilon_{s_4})]e^{-\frac{\alpha}{\mu(x^*(y_1)-l)}} \\
    \end{aligned}
\end{equation}

Since $\epsilon_{s_1}, \epsilon_{s_4} < \delta$, we find a $\delta'$ small enough such that the equation above is positive. This means that each term in $\Delta_{S_4}$ is strictly larger than its corresponding term in $\Delta_{S_1}$. Therefore, we have
\begin{equation}\label{s14}
    \Delta_{S_1} + \Delta_{S_4} > 0    
\end{equation}

By similar argument, we can find a $\delta''$ small enough such that
\begin{equation}\label{s23}
    \Delta_{S_2} + \Delta_{S_3} > 0    
\end{equation}

Now, let's consider the last interval $S_5$
\begin{equation*}
    \begin{split}
        \Delta_{S_5} &= \sum_{z \in N(S_5)} [B(y_1|z)-B(y_2|z)]e^{-\frac{\alpha}{\mu(y_c|z)}} 
    \end{split}
\end{equation*}
Since $y_1$ is closer to agents in $N(S_5)$ than $y_2$ by construction, we have 
$$B(y_1|z) > B(y_2|z) \text{  ,   } \forall z \in N(S_5)$$
This immediately leas to, 
\begin{equation}\label{s5}
    \Delta_{S_5} > 0
\end{equation}

Combining the results, let $\delta = min\{\delta',\delta''\}$, we have 
$$\Delta_{S_1}+\Delta_{S_2}+\Delta_{S_3}+\Delta_{S_4}+\Delta_{S_5}>0$$
Therefore, we obtain 
\begin{equation*}
    \sum_{z \in \Com \backslash \{y_1\}} B(y_1|z)e^{\frac{-\alpha}{\mu(y_c|z)}}> \sum_{z \in \Com \backslash \{y_2\}} B(y_2|z)e^{\frac{-\alpha}{\mu(y_c|z)}}
\end{equation*}


\end{proof}

==> content/lemma/lemmaperiphery_agent_allocation.tex <==
\begin{lemma}\label{lemma:periphery_agent_allocation}
Let $b_{min} = \max \{ b^1, b^2\}$
If 
$$b_0 > b_{min}$$
then for all agents $y_i, y_j$ in the community, if 
$$\|y_i - \Icen \| < \|y_j - \Icen \|$$
then we have 
$$\mu(y_0|y_i) > \mu(y_0|y_j)$$
\end{lemma}

\begin{proof}
Let $y_i, y_j$ be any two agents in the community. Without loss of generality, we assume that
$$\|y_i - y_0\|<\|y_j - y_0\|$$
Since $b_0 > b^1$, by Lemma \ref{lemma:bmin1}, we have that $S(y_0|y_i) > S(y_0|y_j)$. Or equivalently,
$$\sum_{z \in \Com \backslash\{y\}}  B(z|y_i) e^{  - \frac{\alpha}{\mu(z|y_0)} } > \sum_{z \in \Com \backslash\{y\}}  B(z|y_j) e^{  - \frac{\alpha}{\mu(z|y_0)} }$$


Recall the partial derivative with respect to $\mu(y_0|y)$ in the optimization is 
$$ \frac{dH(\mu(y))}{d\mu(y_0|y)}=\frac{\alpha}{\mu^2(y_0|y)}e^{ - \frac{\alpha}{\mu(y_0|y)}} S(y_0|y)$$
For the allocation to be optimal, the allocation need to satisfy the first order condition. By lemma \ref{lemma:bmin2}, we have that for all agent periphery agents $y$, $\mu(y_0|y) > 0$. This means that the first order condition with respect to $\mu(y_0|y)$ is $\frac{dH(\mu(y))}{d\mu(y_0|y)} = \beta$. Because $\beta$ is same for all agents, we have 

\begin{equation}
    \begin{split}
         \frac{\alpha}{\mu^2(y_0|y_i)}e^{ - \frac{\alpha}{\mu(y_0|y_i)}}  S(y_0|y_i)
        = 
         \frac{\alpha}{\mu^2(y_0|y_j)}e^{ - \frac{\alpha}{\mu(y_0|y_j)}}  S(y_0|y_j)
    \end{split}
\end{equation}

Since $\|y_i - \Icen \| < \|y_j - \Icen \|$ by assumption, by lemma \ref{lemma:bmin1}, we have
\begin{equation}
    S(y_0|y_i) > S(y_0|y_j)
\end{equation}
This leads to
$$\mu(y_0|y_i) > \mu(y_0|y_j)$$
\end{proof}

==> content/lemma/lemmaperiphery_respond.tex <==
\newpage
\begin{lemma}\label{lemma:periphery_respond}
	If the allocation of core agent $y_c$ has the property that
	for agents $y_1, y_2$ in the community such that
	$$\mu(y_1|y_c) > \mu(y_2|y_c)$$
	if 
	$$\|y_1 - \Icen \| < \|y_2 - \Icen \|$$
	then, there exist a constant $\delta_1$, if the community density $\delta < \delta_1$, we have
	$$\mu(y_c|y_1) > \mu(y_c|y_2)$$
\end{lemma}

\begin{proof}
	Let $y_1$, $y_2$ be two arbitrary agents such that 
	$$\|y_1-y_c\| < \|y_2-y_c\|$$
	To show the result of this lemma, it is enough to show the following
	\begin{equation}
		S(y_c|y_1) > S(y_c|y_2)
	\end{equation}
	or equivalently
	\begin{equation}\label{eq:sufficient_condition}
	\sum_{z \in \Com \backslash \{y_1\}} B(y_1|z)e^{\frac{-\alpha}{\mu(z|y_c)}}> \sum_{z \in \Com \backslash \{y_2\}} B(y_2|z)e^{\frac{-\alpha}{\mu(z|y_c)}}
	\end{equation}
	then, first order condition condition would imply the optimal allocation has 
	$$\mu(y_1|y_c) > \mu(y_2|y_c)$$
	
	
	Recall $\delta$ is the distance of any consecutive agents in the content space of the community and it determine the community density. As $\delta$ decrease, the community density increase.
	In addition, under the case without delay, by Proposition \ref{prop:benefit_rank}, we have that 
	$ \sum_{z \in \Com \backslash \{y_1\}} B(z|y_1)> \sum_{z \in \Com \backslash \{y_2\}} B(z|y_2)$. Therefore, this lemma aim to establish that under the condition described, this relation is also true for the case with delay. Using these results, we partition the community content interval and compare the utility of agents in each section. We will see that so long as the community is dense enough ($\delta$ small enough), then we obtain the relation in equation \ref{eq:sufficient_condition}.
	
	
	Let $\mu^*(y_c)$ be the rate allocation vector of core agents with the property described in the Lemma. Without loss of generality, let's assume that content interval of the community is given by the following
	$$I_C = (-L_C, L_C) \mbox{ and } mid(I_C) = 0$$
	Then$\|y_1-\Icen \| < \|y_2-\Icen \|$ leads to three possible cases:\\
	case 1: $y_1$ and $y_2$ are in the same side of the community, (0,$L_C$)\\
	case 2: $y_1$ and $y_2$ are in the same side of the community, ($-L_C$,0)\\
	case 3: $y_1$ and $y_2$ are on different side of the community
	
	
	The proof for these three cases are similar. Therefore, we will only construct proof for one of the case above. Let's consider the case $y_1$, and $y_2$ are on the same half interval, (0,$L_C$). We can partition the community interval into the following sections:\\
	
	
	\begin{equation*}
	\begin{split}
	S_1 &= (y_2,L_C)\\
	S_2 &= (\frac{y_2+y_1}{2},y_2)\\
	S_3 &= (y_1,\frac{y_2+y_1}{2})\\
	S_4 &= (y_1+y_2-L_C,y_1)\\
	S_5 &= (-L_C,y_1+y_2-L_C)
	\end{split}
	\end{equation*}
	
	
	Then, let's consider the difference of utility in each sections above.\\
	Let $N(S_i)$ denote the set of contents in the interval $S_i$, $\|N(S_i)\|$ is the number of content in $S_i$, and let $\Delta_{S_i}$ denote the difference of utility between $y_1$ and $y_2$ in interval $S_i$. To simply the notation, 
	let $g(z)$ denote the rate of content produce is produced in the content. $g(z)$ is equivalent to $g(z|y)$ where $y$ is the producer of content $z$. Furhter, let 
	$\mu(z)$ denote the rate core agent allocate for the agent that produce content $z$. $\mu(z)$ is equivalent $\mu(y|y_c)$ where $y$ is the producer of content $z$.  Then, the $\Delta_{S_i}$ is given by 
	
	\begin{equation*}
	\begin{split}
	\Delta_{S_i} &=\sum_{z \in N(S_i)} g(z)[f(z|y_1)-f(z|y_2)] e^{-\frac{\alpha}{\mu(y_c|z)}} \\
	\end{split}
	\end{equation*}
	
	
	We will show that the overall difference of $\Delta_{S_4}$ and $\Delta_{S_1}$ is positive,i.e,
	$$\Delta_{S_4} + \Delta_{S_1} > 0$$
	
	By Proposition \ref{prop:production_strategy}, we know that the distance between consecutive contents is the smaller(higher density) on the interval $S_4$ than $S_1$, and by construction, we have
	$$\|S_1\| = \|S_4\|$$
	which implies 
	$$\|N(S_1)\| < \|N(S_4)\|$$
	Let $J = \|N(S_1)\|, K = \|N(S_4)\|$. Further, let $\{d_i\}_{i \in J}$ be the set of distance between content in $S_1$ to agent $y_1$ in increasing order,i.e, $d_i < d_{i+1}$. Similarly, let $\{s_j\}_{j \in K}$ be the set of distance between content in $S_4$ to agent $y_2$. We can rewrite $\Delta_{S_1}$ and $\Delta_{S_4}$ as
	
	 
	\begin{equation}\label{eq:s1_consumption}
	\begin{split}
	\Delta_{S_1} &= - \sum_{i=1}^J g(y_2 + d_i)[f(d_i)-f(y_2 - y_1 + d_i) ]e^{-\frac{\alpha}{\mu(y_2 + d_i)}}
	\end{split}
	\end{equation}
	
	
	\begin{equation}\label{eq:s4_consumption}
	\begin{split}
	\Delta_{S_4} &= \sum_{k=1}^K g(y_1 - s_k)[f(s_k)-f(y_2 - y_1 + s_k)]e^{-\frac{\alpha}{\mu(y_1 - s_k)}}
	\end{split}
	\end{equation}
	
	Then, with the result from Proposition \ref{prop:production_strategy}, we have 
	
	\begin{equation}
		g(y_2 + d_i) < g(y_1 - s_k) \forall d_i, s_k
	\end{equation}

	and by assumption of this proposition, we have that
	
	\begin{equation}
		e^{-\frac{\alpha}{\mu(y_2 + d_i)}} <e^{-\frac{\alpha}{\mu(y_1 - s_k)}} \forall d_i, s_k
	\end{equation}
	
	
	Let's consider $d_i$ and $s_i$ for $i \in J$. Because that distance of consecutive content item in $S_4$ is strictly less than $S_1$ as we established earlier. This lead to $d_i > s_i$ for $i \in J$. This means that for all $i \in J$, we can write $d_i$ as following
	
	
	\begin{equation}
		d_i  = s_i  + \epsilon_i
	\end{equation}
	
	where $\epsilon_i < \delta$
	
	Using this, and the convexity of $f$ function we can rewrite the term in Eq. \eqref{eq:s1_consumption} as
	\begin{equation}
		\begin{aligned}
			f(d_i) &- f(y_2 - y_1 + d_i) \\
			&=  f(s_i + \epsilon_i) - f(y_2 - y_1 + s_i + \epsilon_i)\\
			&\text{(first order condition of convex function)}\\
			&\leq f(s_i) - f(y_2 - y_1 + s_i) + \epsilon_i 
		\end{aligned}
	\end{equation}
	
%	Then, let's split 
%	let's consider the difference between the first $J$ term in Eq. \eqref{eq:s4_consumption} and Eq. \eqref{eq:s1_consumption}. For each term in this difference, we have that 
	
	With this, let's rewrite the sum of $\Delta_{S_4} + \Delta_{S_1}$
	
	\begin{equation}
		\begin{aligned}
			&\Delta_{S_4} + \Delta_{S_1} =\\
			& \sum_{k=1}^K g(y_1 - s_k)[f(s_k)-f(y_2 - y_1 + s_k)]e^{-\frac{\alpha}{\mu(y_1 - s_k)}} \\
			&- \sum_{i=1}^J g(y_2 + d_i)[f(d_i)-f(y_2 - y_1 + d_i) ]e^{-\frac{\alpha}{\mu(y_2 + d_i)}}\\
			& = \\
			&\sum_{k=J}^K g(y_1 - s_k)[f(s_k)-f(y_2 - y_1 + s_k)]e^{-\frac{\alpha}{\mu(y_1 - s_k)}} \\
			& + \sum_{i=1}^J g(y_1 - s_i)[f(s_i)-f(y_2 - y_1 + s_i)]e^{-\frac{\alpha}{\mu(y_1 - s_i)}}\\
			& - \sum_{i=1}^J g(y_2 + d_i)[f(d_i)-f(y_2 - y_1 + d_i) ]e^{-\frac{\alpha}{\mu(y_2 + d_i)}}\\			
			&>\\
			& \sum_{k=J}^K g(y_1 - s_k)[f(s_k)-f(y_2 - y_1 + s_k)]e^{-\frac{\alpha}{\mu(y_1 - s_k)}} \\
			& + \sum_{i=1}^J [g(y_1 - s_i)e^{-\frac{\alpha}{\mu(y_1 - s_i)}} - g(y_2 + d_i)e^{-\frac{\alpha}{\mu(y_2 + d_i)}}]*\\
			&(f(s_i)-f(y_2 - y_1 + s_i))\\
			& - O(\delta)
		\end{aligned}
	\end{equation}
	
	\begin{equation}
		\begin{aligned}
		\sum_{k=J}^K g(y_1 - s_k)[f(s_k)-f(y_2 - y_1 + s_k)]e^{-\frac{\alpha}{\mu(y_1 - s_k)}}  > 0 
		\end{aligned}
	\end{equation}

	\begin{equation}
	\begin{aligned}
	&\sum_{i=1}^J [g(y_1 - s_i)e^{-\frac{\alpha}{\mu(y_1 - s_i)}} - g(y_2 + d_i)e^{-\frac{\alpha}{\mu(y_2 + d_i)}}]*\\
	&(f(s_i)-f(y_2 - y_1 + s_i)) > 0\\
	\end{aligned}
	\end{equation}
	
	Therefore, we can a find $\delta'$ small enough so that the negative term is bounded by the sum of these two terms. This leads to
	\begin{equation}\label{s14}
	\Delta_{S_1} + \Delta_{S_4} > 0    
	\end{equation}
	
	
	By similar argument, we can find a $\delta''$ such that 
	\begin{equation}\label{s23}
	\Delta_{S_2} + \Delta_{S_3} > 0    
	\end{equation}
	
	
	For the last interval $S_5$
	\begin{equation*}
	\begin{split}
	\Delta_{S_5} &= \sum_{z \in N(S_5)} g(z)[f(z|y_1)-f(z|y_2)]e^{-\frac{\alpha}{\mu(z)}} 
	\end{split}
	\end{equation*}
	
	Since $y_1$ is closer to content in $N(S_5)$ than $y_2$ by construction, we have 
	$$f(z|y_1) > f(z|y_2) \text{  ,   } \forall z \in N(S_5)$$
	This immediately leas to, 
	\begin{equation}\label{s5}
	\Delta_{S_5} > 0
	\end{equation}
	
	Combining the results above and let $\delta_1 = min\{\delta', \delta''\}$ above, we get
	$$\Delta_{S_1}+\Delta_{S_2}+\Delta_{S_3}+\Delta_{S_4}+\Delta_{S_5}>0$$
	Therefore, we obtain 
	\begin{equation*}
	\sum_{z \in \Com \backslash \{y_1\}} B(z|y_1)e^{\frac{-\alpha}{\mu(y_c|z)}}> \sum_{z \in \Com \backslash \{y_2\}} B(z|y_2)e^{\frac{-\alpha}{\mu(y_c|z)}}
	\end{equation*}
	or equivalent 
	\begin{equation*}
	S(y_c|y_1)> S(y_c|y_2)
	\end{equation*}
	
	
\end{proof}

==> content/lemma/lemmasufficient_budget1.tex <==
\begin{lemma}\label{lemma:bmin1}
There exist a finite positive $b^1$ such that if the budget of core agent $b_0 > b^1$, then agent, closer to the center of community, would benefit more from the content of core agent. In other word, given two leaf agents $y_i, y_j$
$$\|y_i - y_0\|<\|y_j - y_0\|$$
we have 
$$S(y_0|y_i) > S(y_0|y_j)$$
\end{lemma}

\begin{proof}
By assumption \ref{assump:benefit_rank}, we have that in the case without delay, agent closer to the center of community would benefit more from the content of the community. More precisely, for agents $y_i,y_j$, if 
$$\|y_i - \Icen \|<\|y_j - \Icen \|$$
then
$$\sum_{z \in \Com \backslash \{y_i\}} B(z|y_i)> \sum_{z \in \Com \backslash \{y_j\}}B(z|y_j)$$
Let
\begin{equation}\label{eq:delta}
    \begin{split}
        &\Delta = \min_{\cb{y_i,y_j| \|y_i - \Icen \| \neq \|y_j - \Icen \|}}\\
        &\hspace{0.5in}  \|\sum_{z \in \Com \backslash \{y_i\}} B(z|y_i) - \sum_{z \in \Com \backslash \{ y_j\}}B(z|y_j)\|
    \end{split}
\end{equation}
In other word, $\Delta$ is the minimum difference of consumption utility of any two agents in the community in the case without delay.


Since the delay factor of core agent getting content from periphery agent $y$ is a monotonic increasing function with respect to the allocation rate $\mu(y|y_0)$, we have $e^{\frac{-\alpha}{\mu(y|y_0)}} \xrightarrow{} 1, \text{ as } \mu(y|y_0) \xrightarrow{} \infty$. This means as the rate allocation increase, we can find a upper bound between the difference of the case with delay and the case without delay for each agent. Let $\epsilon_{y}$ be the upper bound of the difference between the case with delay and the case without delay for agent $y$. In other word, let 


\begin{equation}
    \epsilon_{y} \geq 1 -  e^{\frac{-\alpha}{\mu(y|y_0)}}
\end{equation}


Then, we can find the maximum difference among all agent. In other word, find the agent that is effected by the delay the most and denote the its delay effect as $\epsilon^*$.  



\begin{equation}\label{eq:epsilon}
    \epsilon^* = \max_{y \in \Com}\epsilon_{y}
\end{equation}


As $b_0 \xrightarrow{} \infty$,  $\epsilon^* \xrightarrow{} 0$. 


Let's denote the number of periphery agent in the community as N. We can find a finite $b^1$ large enough such that $\Delta > N\epsilon^*$. Then, for all periphery agent $y_i,y_j$ in the community, we have 
\begin{equation}
    \begin{split}
        \sum_{z \in \Com \backslash \{y_i\}} B(z|y_i)e^{\frac{-\alpha}{\mu(z|y_0)}} - \sum_{z \in \Com \backslash \{y_j\}}B(z|y_j)e^{\frac{-\alpha}{\mu(z|y_0)}} &> \Delta \\
        & > N\epsilon^*
    \end{split}
\end{equation}
By equation\ref{eq:delta} and equation \ref{eq:epsilon}, we have 
\begin{equation}
    \begin{split}
        S(y_0|y_i) &> \sum_{z \in \Com \backslash \{y_i\}} B(z|y_i)e^{\frac{-\alpha}{\mu(z|y_0)}} - N\epsilon^* \\
        &> \sum_{z \in \Com \backslash \{y_j\}}B(z|y_j)e^{\frac{-\alpha}{\mu(z|y_0)}}\\
        &>S(y_0|y_j)
    \end{split}
\end{equation}

Therefore, we have 
$$S(y_0|y_i) > S(y_0|y_j)$$

\end{proof}


==> content/lemma/lemmasufficient_budget2.tex <==
\begin{lemma}\label{lemma:bmin2}
For all agent y in the community, let $z^*_y = \max_z B(z|y)$. In other word, $z^*_y$ is the agent that produce content is of most beneficial to agent y. 


There exist a finite positive $b^2$ such that if the budget of core agent $b_0 > b^2$, we have
$$S(y_0|y) > B(z^*_y|y)$$
This means that the core agent possess content is of the highest value to agent y.
\end{lemma}

\begin{proof}
In the case without delay, for all agent y in the community we have that 
$$\sum_{z \in \Com \backslash \cb{y}} B(z|y)> B(z^*_y|y) $$
Let $\Delta = \min_{y \in \Com} \sum_{z \in C \backslash \{y\}} B(z|y) - B(z^*|y)$. In other word, $\Delta$ is the minimum difference between the total utility of whole community content and utility of the highest valuable content for any agent in the community. 

As we establish in the proof of lemma \ref{lemma:bmin1}, for all positive $\epsilon$, we can find a positive finite $b^2$ large enough such that 
$$\sum_{z \in \Com \backslash \cb{y}} B(z|y) - S(y_0|y) < \epsilon$$
Therefore, we can make $b^2$ large enough such that we have $\epsilon < \Delta$. This leads to that for all agent y we have,
\begin{equation*}
    \begin{split}
        \sum_{z \in \Com \backslash \cb{y}} B(z|y) - S(y_0|y) &< \epsilon \\
        &<\Delta\\
        &\leq \sum_{z \in \Com \backslash \cb{y}} B(z|y) - B(z^*_y|y)
    \end{split}
\end{equation*}
Therefore, if $b_0 > b^2$, then we have for any agent y, 
$$S(y_0|y) > B(z^*_y|y)$$


\end{proof}

==> content/math_model.tex <==
\section{Mathematical Model}\label{sec:model}
We consider a group of users who share a common interest, where we assume that there are several different topics (viewpoints) associated with this common interest. While users are  interested in several (or all) of these topics (viewpoints), we assume that each user has a main interest, i.e. each users has a topic in which they are most interested in.
In addition, we assume that users have a different range of interests, where some users are interested in a narrow set of topics, and other users are interested in a broad set of topics.

For this setting, we study how content recommendation algorithms impact the user population who are active on a social media platform, where we characterize this popluation by the corresponding distribution of users with narrow and broad interests.
%To do this, we assume that there is a set users who are content producers, and a set of users are content consumers.
To do that, we use the following model.






\noindent{\underline{Topics of Interest $\setT$:}}
We consider a group of users consisting of a set of content producers $\setP$, and a set of content consumers $\setC$. We characterize the content that users in the group are interested by a set of topics $\setT$ given by $\setT=(T_{-M},...,T_M)$.
We model the topics of interest $\setT$ as follows.
We assume that the set of topics $\setT$ is ordered in such a way that two topics that are close to each other in this order, are also more closely thematically related with each other.
In addition, we assume that content producers in the group create (post) content that can be associated with one of these topics. That is, each content item is on a specific  topic $T \in \setT$.

We use a parameter $a \geq 0$ to characterize the range of interest of a user. For our analysis, we assume that set of  parameters $a$ is given by a discrete set $\setA$. We define more precisely how we use the parameter in the following. 

\noindent{\underline{Content Producers:}}
We characterize content producers in the set $\setP$ by two variables: a) their main interest $i \in \setT$, and the range of their interest given by the parameter $a \geq 0$. 
To do that, we first associate with each content producer a main interest $i \in \setT$ which is the topic for which they are most adapt at creating content. 
Let $\setP_i$, $i=-M,...,M$,  be the set of content producers  whose main interest is topic $T_i$. We assume that the number of content producers whose main interest is a given topic $T \in \setT$ is the same, and equal to $N_p$.

Content producers can create content on  other topics, however the further away the topic is from their main interest, the lower is the quality of the content that they produce for this topic.
We model this as follows.
Given a content producer $x \in \setP_i$ with main interest $i \in \setT$, and range of interest $a \in \setA$, the (average) quality $q(k|a,i)$ of content on topic $T_k$ that the producer creates $x$  is given by
$\funq{a}{i}(k) = \funf{a}(|k-i|)$,
where
$$\funf{a}(|k-i|) = \max\{0, \fo{a} - a|k-i|\}.$$
Note that this function captures the intuition that the content producer  $x \in \setP_i$ creates  higher quality content item on topics that are closer to its main interest $T_i$.

We have that
$$\funf{a}(0) = \kappa(a).$$

Let $N_p(a)$ be the number of content producers with main interest $i$ and interest-range $a$, and we have that $\sum_{a \in \setA} N_P(a) = N_P$. 

Content producers can decide on which topics they produce content, and we denote with $\cprod{a}{i}(i)$ the amount of content (number of content items) created by a content producers $x \in \setP_i$ with range of interest $a$. 
We assume that  that there is a bound (capacity) of the number of content items that a producer can create within a given time period, and we have that
$$\sum_{k=-M}^M{\cprod{a}{i}(k)} \leq L_p, $$
where $L_p > 0$. We refer to $L_p$  as the production capacity.


\noindent{\underline{ Content Consumers:}}
We model content consumers, and their interest in content on the different topics $T \in \setT$ as follows.
Each consumer has a main interest which is given by one of the topics $T \in \setT$. Let $\setC_i$, $i=-M,...,M$,  be the set of content consumers  whose main interest is topic $T_i$. To simplify the notation and analysis, we assume that the number of content consumers whose main interest is a given topic $T \in \setT$ is the same, and equal to $N_c$, for all topics, i.e. we have that $|\setC_i| = N_c$,  $i=-M,...,M$.

Consumers are also interested in topics other than their main interest; however the further away the topics is from their main interest, the less likely it is that they find a content item on this topic to be of interest to them.
Let $\funp{b}{j}(k)$ denote the interest (factor) of content consumer $c \in \setC_i$ in content items on topic $T_k$. We assume that $\funp{b}(k|j)$ is given by
$\funp{b}{j}(k) = \funf{b}(|k-j|)$,
where the function $\funf{b}: \{0, 1, \ldots, 2M\} \to [0, 1]$ is as defined by Eq.~\eqref{..}. 



